TEMPO: Semantic-Action Decoupled RL Post-Training for Vision-Language-Action Models

Vision-language-action (VLA) models are commonly adapted to downstream manipulation tasks via supervised fine-tuning (SFT) or online reinforcement learning(RL) post-training. SFT is prone to distribution mismatch, and existing RL approaches typically optimize all trainable components within a single RL loop at a uniform update rate, although these components play distinct functional roles. We propose TEMPO, a semantic-action decoupled, two-timescale RL post-training framework for VLA models. TEMPO freezes the pretrained vision-language backbone and adapts two components with dedicated RL loops: the semantic projection layer, which produces the latent action conditioning the action expert, and the low-level action expert itself. The semantic projection layer is updated infrequently and the action expert frequently, which aims to limit latent-action drift while allowing the action expert to learn from online feedback. Our analyses show that, compared with equal update frequencies, less frequent semantic updates reduce latent-action drift and improve policy performance. Experiments on the CALVIN benchmark and real-world manipulation tasks demonstrate that TEMPO outperforms both pretrained state-of-the-art VLA models and the RL post-training baseline, while reaching and maintaining higher evaluation rewards on three real-world tasks.

==> tempo_response_figures/replay_mismatch_legend.tex <==
\definecolor{ratioone}{RGB}{53,118,173}
\definecolor{ratiotwo}{RGB}{209,133,39}
\definecolor{ratiothree}{RGB}{32,136,113}
\definecolor{ratiofour}{RGB}{172,81,117}
\definecolor{ratiofive}{RGB}{117,103,173}
\newcommand{\replaymismatchplot}[1]{%
\resizebox{#1}{!}{%
\begin{tikzpicture}
\node[anchor=south west,inner sep=0pt] (plot) at (0,0) {\includegraphics[width=10cm,trim=0 27bp 0 0,clip]{tempo_response_figures/replay_mismatch.png}};
\begin{scope}[x={(plot.south east)},y={(plot.north west)}]
\draw[ratioone,line width=1.0pt] (0.145,0.915) -- (0.180,0.915);
\node[anchor=west,inner sep=0pt,font=\fontsize{8}{9}\selectfont] at (0.195,0.915) {1:1};
\draw[ratiotwo,line width=1.0pt] (0.145,0.860) -- (0.180,0.860);
\node[anchor=west,inner sep=0pt,font=\fontsize{8}{9}\selectfont] at (0.195,0.860) {2:1};
\draw[ratiothree,line width=1.0pt] (0.145,0.805) -- (0.180,0.805);
\node[anchor=west,inner sep=0pt,font=\fontsize{8}{9}\selectfont] at (0.195,0.805) {3:1};
\draw[ratiofour,line width=1.0pt] (0.145,0.750) -- (0.180,0.750);
\node[anchor=west,inner sep=0pt,font=\fontsize{8}{9}\selectfont] at (0.195,0.750) {4:1};
\draw[ratiofive,line width=1.0pt] (0.145,0.695) -- (0.180,0.695);
\node[anchor=west,inner sep=0pt,font=\fontsize{8}{9}\selectfont] at (0.195,0.695) {5:1};
\end{scope}
\end{tikzpicture}%
}%
}

